Multi-Wideband Terahertz Communications via Tunable Graphene-based Metasurfaces in 6G Networks

The next generation of wireless networks is expected to tap into the terahertz (0.1--10 THz) band to satisfy the extreme latency and bandwidth density requirements of future applications. However, the development of systems in this band is challenging as THz waves confront severe spreading and penetration losses, as well as molecular absorption, which leads to strong line-of-sight requirements through highly directive antennas. Recently, reconfigurable intelligent surfaces (RISs) have been proposed to address issues derived from non-line-of-sight propagation, among other impairments, by redirecting the incident wave toward the receiver and implementing virtual-line-of-sight communications. However, the benefits provided by a RIS may be lost if the network operates at multiple bands. In this position paper, the suitability of the RIS paradigm in indoor THz scenarios for 6G is assessed grounded on the analysis of a tunable graphene-based RIS that can operate in multiple wideband transparency windows. A possible implementation of such a RIS is provided and numerically evaluated at 0.65/0.85/1.05 THz separately, demonstrating that beam steering and other relevant functionalities are realizable with excellent performance. Finally, the challenges associated with the design and fabrication of multi-wideband graphene-based RISs are discussed, paving the way to the concurrent control of multiple THz bands in the context of 6G networks.

==> background.tex <==
\hl{A bit of deeper intro and state of the art in the different facets of the work.}\textcolor{red}{Odysseas and Ana}
\\
\\
\\
%\subsection{The Distance Problem at mmWave-THz Bands}
\hl{Comment the main aspects relative to the distance problem, wireless comms oriented.}
\cite{akyildiz2018combating}\textcolor{red}{Odysseas}
\\
\\
\\
%\subsection{Reconfigurable Intelligent Surfaces for Wireless Communications}
\hl{Describe the existence of prototypes for RIS, wireless comms oriented.}\textcolor{red}{Odysseas and Sergi}
\\
\\
\\
%\hl{2) Mention that their application for wireless are endless, but provide a short summary of most prominent works on the area of RIS for wireless communications.}

\hl{Briefly describe how those can help to address the distance problem.}\textcolor{red}{Odysseas}
\\
\\
\\
\hl{Mention that there is not much work specific for mmWave-THz frequencies. We are different and aim to bridge this gap.}\textcolor{red}{Odysseas}

%\subsection{Programmable Metasurfaces at mmWave-THz Frequencies}
%\hl{Definition of metasurface and programmable. Mention that programmable metasurfaces are expected to be a crucial component within RIS. Demonstration at mmWave-THz bands (especially THz) is still uncertain. We bridge this gap.}

\cite{tsilipakostoward, abadal2020programmable}

\cite{pitchappa2020frequency}
\\
\\
\\
\hl{Mention that graphene-based metasurfaces are the excellent candidate at mmWave-THz bands (especially THz) }\textcolor{red}{Ana}

\cite{Correas2017}
\cite{han2020complete}
\cite{cheng2019recent}

==> comms.tex <==
\hl{Description of the communications architecture from Fig. 1, in more detail. The metasurface could indeed have a gateway that connects to APs/BSs to coordinate their actions and look for the best options in terms of propagation/modulation and so on. Description of the possible protocols and algorithms involved.}

==> results.tex <==
Fig.~\ref{fig:codings} shows the pattern resulting from the reflection of a normally incident plane-wave to \hl{insert 2-3 distinct angles} for \hl{insert the 3 frequencies evaluated in the paper}.\textcolor{red}{Hamidreza}
\\
\\
\\
\begin{figure}[!ht]
    \centering
    \includegraphics[width=\columnwidth,height=3cm]{example-image-a}
    \caption{Reflection patterns for metasurface codings pointing at \hl{insert 2-3 distinct angles} for \hl{insert the 3 frequencies evaluated in the paper}.}\label{fig:codings}
\end{figure}
\\
\\
\\
%\subsection*{Capacity Analysis}

%\hl{Tentative sub-section.}


%\subsection*{????}

%\hl{Tentative sub-section.}


%\subsection*{Impact of Low-Quality Graphene}
%The unit cell design relies on the use of high-quality graphene with reasonably high carrier mobility, and thus high relaxation time, which results in low losses in the THz band. However, this is an assumption that hinges on the availability of manufacturing and integration processes that are capable of achieving such conditions. While high-quality graphene manufacturing has been demonstrated experimentally in multiple works \cite{Banszerus2015}, device-level integration has still some pending challenges \cite{illarionov2020insulators}. Thus, it is pertinent to explore the performance of the proposed solution for lower graphene qualities. To this end, we next show a cross-cutting evaluation for different values of relaxation time.
\section{Discussion}
\hl{Metasurface: how frequency modulation affects directivity and other metrics.}\textcolor{red}{Hamidreza and Alex}

